Socially Acceptable Bipedal Robot Navigation via Social Zonotope Network Model Predictive Control

This study addresses the challenge of social bipedal navigation in a dynamic, human-crowded environment, a research area largely underexplored in legged robot navigation. We present a zonotope-based framework that couples prediction and motion planning for a bipedal ego-agent to account for bidirectional influence with the surrounding pedestrians. This framework incorporates a Social Zonotope Network (SZN), a neural network that predicts future pedestrian reachable sets and plans future socially acceptable reachable set for the ego-agent. SZN generates the reachable sets as zonotopes for efficient reachability-based planning, collision checking, and online uncertainty parameterization. Locomotion-specific losses are added to the SZN training process to adhere to the dynamic limits of the bipedal robot that are not explicitly present in the human crowds data set. These loss functions enable the SZN to generate locomotion paths that are more dynamically feasible for improved tracking. SZN is integrated with a Model Predictive Controller (SZN-MPC) for footstep planning for our bipedal robot Digit. SZN-MPC solves for collision-free trajectory by optimizing through SZN's gradients. and Our results demonstrate the framework's effectiveness in producing a socially acceptable path, with consistent locomotion velocity, and optimality. The SZN-MPC framework is validated with extensive simulations and hardware experiments.

==> bio.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/aziz.png}}]{Abdulaziz Shamsah}
received B.S. in mechanical engineering from Rensselaer Polytechnic Institute. Troy, NY, USA in 2016, and the M.S.E degree in mechanical engineering and applied mechanics from the University of Pennsylvania, Philadelphia, PA, USA in 2018.

Currently, he is pursuing a Ph.D. degree in mechanical engineering at the Georgia Institute of Technology in Atlanta, GA, USA. In 2019, he was awarded a fellowship from Kuwait University, Kuwait.

His research interest includes bipedal navigation in real-world environments, formal methods, and safety and robustness in locomotion.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/krishanu.png}}]{Krishanu Agarwal}
received B.Tech in Mechatronics from Manipal University Jaipur, Jaipur, Rajasthan, India in 2021 and M.S. degree in Robotics from Georgia Institute of Technology, Atlanta, GA, USA in 2024.

His research interests includes Robot learning, Path planning, Generative AI and safety in locomotion. 
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/nigam.png}}]{Nigam Katta}
received B.Tech in electronics and communication engineering from Amrita Vishwa Vidyapeetam, Amritapuri, Kerala, India in 2020 and M.S. degree in Robotics from the Georgia Institute of Technology, Atlanta, GA, USA in 2024.

His research interests include Computer Vision, photogrammetry, and bipedal robot navigation.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/abirath.png}}]{Abirath Raju}
received B.Tech in mechanical engineering with a minor in computer science from the National Institute of Technology, Tiruchirappalli, Tamil Nadu, India in 2023.

Currently, he is pursuing an M.S. degree in Robotics at the Georgia Institute of Technology, Atlanta, GA, USA. 

His research interests include computer vision, bipedal robot navigation, and robot learning.


\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/shreyas.png}}]{Shreyas Kousik} (Member, IEEE) received the B.S. degree in mechanical engineering from the Georgia Institute of Technology, Atlanta, GA,
USA, in 2014, and the M.S. and Ph.D. degrees in mechanical engineering from the University of Michigan, Ann Arbor, MI, USA, in 2020.
He was a Postdoctoral Scholar at Stanford University, Stanford, CA, USA.
He is currently an Assistant Professor with the George W. Woodruff School of Mechanical Engineering, Georgia Institute of Technology, Atlanta, GA, USA. His research interests include safety for full-stack robot autonomy.

\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/ye.png}}]{Ye Zhao} (Senior Member, IEEE) received the Ph.D. degree in mechanical engineering from The University of Texas at Austin, Austin, TX, USA, in 2016. He was a Post-Doctoral Fellow with the John A. Paulson School of Engineering and Applied Sciences, Harvard University, Cambridge, MA, USA. He is currently an Assistant Professor with the George W. Woodruff School of Mechanical Engineering, Georgia Institute of Technology, Atlanta, GA, USA. His research interests include robust task and motion planning, contact-rich trajectory optimization, formal methods for legged locomotion and navigation.

Dr. Zhao serves as an Associate Editor of IEEE Transactions on Robotics (TRO), IEEE Robotics and Automation Letters (RA-L) and IEEE Control Systems Letters (L-CSS). He is a Co-Chair of the IEEE Robotics and Automation Society (RAS) Technical Committee on Whole-Body Control and was a Co-Chair of the IEEE RAS Student Activities Committee. Dr. Zhao received a CAREER Award from the National Science Foundation in 2022 and a Young
Investigator Award from the Office of Naval Research in 2023.

\end{IEEEbiography}

